The Supercluster-Void Network I. The Supercluster Catalogue and Large-Scale Distribution

We investigate the distribution of superclusters and voids using a new catalogue of superclusters of rich clusters of galaxies which extends up to a redshift of z=0.12. The new catalogue contains 220 superclusters of rich clusters, of which 90 superclusters have been determined for the first time. Two thirds of those superclusters with eight or more member clusters are concentrated to a Dominant Supercluster Plane almost perpendicular to the plane of the Local Supercluster. Several independent methods indicate consistently the presence of a quite regular supercluster-void network with scale of approx. 120 Mpc. We determine the selection function of the sample of clusters and suggest that the mean true space density of Abell clusters is 2.6 x 10^-5 h^3 Mpc^-3, or twice the conventionally used value.

==> sc96a1.tex <==
\magnification=800
\looseness=2
\def\msn{\par\nobreak\noindent}
\def\noi{\noindent}
\font\small=cmr8
\baselineskip=14pt plus2pt minus1pt
\parskip=2pt plus1pt minus1pt
%\vglue 0.2truein\noi
\nopagenumbers
\baselineskip=8pt plus1pt minus1pt
\noi
{\bf Appendix}
\msn
{\bf Table~ A1.} The list of rich superclusters (multiplicity $k\geq4$)
$$\vbox
{\small
{\tabskip=0.05truecm
\halign to \hsize { \hfil# &  \hfil# &\hfil# &\hfil#
& \hfil# &
\quad \hfil# \quad& \hfil# \quad&\hfil#\quad &\hfil#\quad&
\hfil# \quad&\hfil# \quad&\hfil# \quad&\hfil# \quad &\hfil# \quad&\hfil# 
& \hfil# & \hfil#
\cr
\noalign {\smallskip}
\noalign{\hrule width 16.4truecm height 0.4pt}
\noalign{\smallskip}
(1)& (2) & (3) & (4) &(5) & &&&&(6)&&&&&&\multispan1 (7) &(8) \cr
\noalign{\smallskip}
$No$& $N_{CL}$&$\alpha_C$&$\delta_C$&$D_C$ 
&&&\multispan4 Abell-ACO No.&&&&&
\multispan1 ID &$N_E$ \cr
  & &  &  &\multispan1$ h^{-1} Mpc$ &&&&&&& & &&&& \cr
\noalign{\smallskip}
\noalign{\hrule width 16.4truecm height 0.4pt}
\noalign {\smallskip}
     3 &     8 &     1.4 &     6.0 &    274 &
     3 &
    16 &
    17 &
  2694 &
2696\rlap{$e$} &
  2698 &
  2700 &
  2706 &
  &
  &
Pegasus - Pisces
  &
1
  \cr
     4 &     4 &     1.9 &   -18.3 &    276 &
    13 &
 2682\rlap{$e$} &
  2710 &
 2756\rlap{$e$} &
  &
  &
  &
  &
  &
  &
Aquarius
&126
  \cr
     5 &     5 &     2.9 &   -35.8 &    327 &
  2715 &
  2721 &
  2730 &
  2767 &
 2772\rlap{$e$} &
  &
  &
  &
  &
  &
&  \cr
     6\rlap{$c$} &     4 &     3.0 &   -62.7 &    299 &
 2732\rlap{$e$} &
 2821\rlap{$e$} &
 4051\rlap{$e$} &
  4067 &
  &
  &
  &
  &
  &
  &
&  \cr
     9 &    22 &     7.3 &   -30.1 &    300 &
    42 &
    88 &
   118 &
   122 &
  2726\rlap{$e$} &
  2751 &
  2755\rlap{$-$} &
  2759\rlap{$e$} &
  2778 &
  2780 &
Sculptor&3
  \cr
 & & & & &
  2798 &
  2801 &
  2804\rlap{$e$} &
  2811 &
  2814 &
  2829 &
  2844 &
  2878\rlap{$e$} &
  4021 &
  4029\rlap{$e$} &
&  \cr
 & & & & &
  4068 &
  4074\rlap{$e$} &
  &
  &
  &
  &
  &
  &
  &
  &
&  \cr
    10 &    17 &     8.6 &   -20.7 &    175 &
    14 &
    27 &
    74 &
    80 &
    85 &
    86 &
    87 &
    93\rlap{$e$} &
   114 &
   117 &
Pisces - Cetus & 6  
  \cr
 & & & & &
   133 &
   151 &
  2716 &
  2734 &
  2800 &
  2824 &
  4053 &
  &
  &
  &
 & 
 \cr
    12\rlap{$c$} &     4 &     9.8 &   -87.7 &    299 &
  2757\rlap{$e$} &
  3037\rlap{$e$} &
  3299\rlap{$e$} &
  3650\rlap{$e$} &
  &
  &
  &
  &
  &
  &
&  \cr
    16 &     4 &    12.5 &   -64.2 &    207 &
  2810\rlap{$e$} &
  2819 &
  2859 &
  2864 &
  &
  &
  &
  &
  &
  &
&15
  \cr
    18 &     6 &    13.2 &   -47.8 &     82 &
  2731 &
  2806 &
  2836 &
  2870 &
  2877 &
  2896 &
  &
  &
  &
  &
Phoenix&8
  \cr
    22\rlap{$c$} &     5 &    15.6 &   -37.7 &    331 &
  2823\rlap{$e$} &
  2838\rlap{$e$} &
  2865\rlap{$e$} &
  2871 &
  2909\rlap{$e$} &
  &
  &
  &
  &
  &
&  \cr
\noalign {\smallskip}
    24 &     7 &    16.9 &     7.6 &    128 &
    76 &
   119 &
   147 &
   160 &
   168 &
   193 &
   195 &
  &
  &
  &
Pisces&16
  \cr
    26\rlap{$c$} &     7 &    19.5 &   -18.6 &    320 &
   166 &
   183 &
   185\rlap{$e$} &
   187\rlap{$e$} &
   197\rlap{$e$} &
   199\rlap{$e$} &
  2866\rlap{$e$} &
  &
  &
  &
&  \cr
    30 &     8 &    23.0 &    17.5 &    190 &
   150 &
   154 &
   158 &
   171 &
   225 &
   257 &
   292 &
   311 &
  &
  &
Pisces - Aries&17
  \cr
    31 &     4 &    24.1 &    -6.6 &    319 &
   216 &
   217 &
   229 &
   243 &
  &
  &
  &
  &
  &
  &
&  \cr
    34 &     6 &    27.7 &    -1.9 &    264 &
   256 &
   266 &
   267\rlap{$e$} &
   268\rlap{$e$} &
   271\rlap{$e$} &
   277 &
  &
  &
  &
  &
  &18
  \cr
    38\rlap{$c$} &     4 &    30.0 &   -26.5 &    330 &
  2944\rlap{$e$} &
  2968\rlap{$e$} &
  2972\rlap{$e$} &
  2981\rlap{$e$} &
  &
  &
  &
  &
  &
  &
&   \cr
    48 &    26 &    48.6 &   -49.3 &    191 &
  3004 &
  3009 &
  3045\rlap{$e$} &
  3074 &
  3078 &
  3089 &
  3093 &
  3100 &
  3104\rlap{$e$} &
  3106 &
Horologium -& 27
 \cr
 & & & & &
  3108 &
  3109 &
  3110 &
  3111 &
  3112 &
  3120 &
  3122 &
  3123 &
  3125 &
  3128 &
 Reticulum&
  \cr
 & & & & &
  3135 &
  3158 &
  3164 &
  3202 &
  3225 &
  3266 &
  &
  &
  &
  &
&
  \cr
    49 &     5 &    48.9 &   -24.9 &    191 &
   419 &
   428 &
  3094 &
  3095 &
  3151 &
  &
  &
  &
  &
  &
&27
  \cr
    50\rlap{$c$} &     6 &    50.0 &   -69.9 &    314 &
  3103\rlap{$e$} &
  3117\rlap{$e$} &
  3119\rlap{$e$} &
  3121\rlap{$e$} &
  3143\rlap{$e$} &
  3155\rlap{$e$} &
  &
  &
  &
  &
&   \cr
    53\rlap{$c$} &    12 &    55.5 &   -32.4 &    290 &
  3118\rlap{$e$} &
  3146 &
  3148\rlap{$e$} &
  3152\rlap{$e$} &
  3153\rlap{$e$} &
  3159\rlap{$e$} &
  3166\rlap{$e$} &
  3171\rlap{$e$} &
  3173\rlap{$e$} &
  3182\rlap{$e$} &
Fornax - Eridanus &28
  \cr
 & & & & &
  3183\rlap{$e$} &
  3194 &
  &
  &
  &
  &
  &
  &
  &
  &
&  \cr
\noalign {\smallskip}
    54\rlap{$c$} &     4 &    57.2 &   -32.1 &    218 &
  3154\rlap{$e$} &
  3161\rlap{$e$} &
  3188\rlap{$e$} &
  3195\rlap{$e$} &
  &
  &
  &
  &
  &
  &
&29
  \cr
    59\rlap{$c$} &    11 &    70.7 &   -33.6 &    298 &
  3253\rlap{$e$} &
  3265\rlap{$e$} &
  3268\rlap{$e$} &
  3273\rlap{$e$} &
  3275\rlap{$e$} &
  3285\rlap{$e$} &
  3289\rlap{$e$} &
  3295 &
  3297 &
  3307\rlap{$e$} &
Caelum &
  \cr
 & & & & &
  3325\rlap{$e$} &
  &
  &
  &
  &
  &
  &
  &
  &
  &
&  \cr
    62 &     5 &    74.3 &     8.5 &    305 &
   515\rlap{$e$} &
   523 &
   525\rlap{$e$} &
   529 &
   532\rlap{$e$} &
  &
  &
  &
  &
  &
&   \cr
    63\rlap{$c$} &     4 &    79.2 &   -49.4 &    314 &
  3303\rlap{$e$} &
  3331\rlap{$e$} &
  3338\rlap{$e$} &
  3361\rlap{$e$} &
  &
  &
  &
  &
  &
  &
&   \cr
    65 &     5 &    83.1 &   -41.3 &    228 &
  3332 &
  3336 &
  3351\rlap{$e$} &
  3360 &
  3379\rlap{$e$} &
  &
  &
  &
  &
  &
&36, 37
  \cr
    66 &     4 &    86.4 &   -21.5 &    262 &
   550\rlap{$e$} &
  3358\rlap{$e$} &
  3365 &
  3368 &
  &
  &
  &
  &
  &
  &
&38, 39
  \cr
    67 &     6 &    88.1 &   -28.1 &    114 &
   548 &
  3341 &
  3367 &
  3374 &
  3381 &
  3390 &
  &
  &
  &
  &
Lepus &41
  \cr
    71 &     5 &   100.9 &    69.5 &    314 &
   554\rlap{$e$} &
   557\rlap{$e$} &
   561\rlap{$e$} &
   562 &
   565 &
  &
  &
  &
  &
  &
&   \cr
    76 &     4 &   131.2 &    28.4 &    244 &
   690 &
   692 &
   699 &
   722 &
  &
  &
  &
  &
  &
  &
&47
  \cr
    82 &     4 &   151.2 &    -0.1 &    265 &
   912 &
   919 &
   933 &
   954 &
  &
  &
  &
  &
  &
  &
&52
  \cr
\noalign {\smallskip}
    88 &     4 &   154.4 &    -7.7 &    159 &
   970 &
   978 &
   979 &
   993 &
  &
  &
  &
  &
  &
  &
Sextans & 53
  \cr
    91 &     9 &   162.6 &     3.0 &    212 &
  1024 &
  1032 &
  1066 &
  1078 &
  1080 &
  1149 &
  1171 &
  1205 &
  1238 &
  &
Vela &58
  \cr
    93 &     9 &   165.2 &    19.9 &     96 &
   999 &
  1016 &
  1139 &
  1142 &
  1177 &
  1185 &
  1228 &
  1257 &
  1267 &
  &
Leo& 56
  \cr
    95 &     4 &   167.6 &    38.6 &    218 &
  1155 &
  1187 &
  1190 &
  1203 &
  &
  &
  &
  &
  &
  &
&55
  \cr
   100 &    10 &   173.7 &    -2.5 &    286 &
  1189\rlap{$e$} &
  1200\rlap{$-$} &
  1248\rlap{$e$} &
  1296\rlap{$e$} &
  1364 &
  1376\rlap{$e$} &
  1386 &
  1389\rlap{$e$} &
  1399\rlap{$-$} &
  1404\rlap{$e$} &
Leo A&64
  \cr
   107 &     8 &   175.9 &    10.0 &    316 &
  1341 &
  1342 &
  1345 &
  1354 &
  1356 &
  1372 &
  1379\rlap{$e$} &
  1435\rlap{$e$} &
  &
 &
Leo - Virgo&
 \cr
   109 &     8 &   176.8 &    54.9 &    173 &
  1270 &
  1291 &
  1318 &
  1377 &
  1383 &
  1436 &
  1452 &
  1507 &
  &
  &
Ursa Majoris &66
  \cr
   111 &    16 &   181.1 &    10.1 &    230 &
  1262 &
  1307 &
  1337 &
  1358 &
  1385 &
  1390 &
  1424 &
  1459 &
  1474 &
  1516 &
Virgo - Coma&70
  \cr
 & & & & &
  1526 &
  1541 &
  1552 &
  1564 &
  1569 &
  1589 &
  &
  &
  &
  &
&  \cr
   114 &    16 &   181.9 &    64.3 &    310 &
  1289 &
  1302 &
  1322 &
  1366 &
  1402 &
  1406 &
  1421 &
  1432 &
  1446 &
  1477 &
Draco&
  \cr
 & & & & &
  1518 &
  1559 &
  1566 &
  1621 &
  1646 &
  1674 &
  &
  &
  &
  &
&  \cr
   115\rlap{$c$} &     5 &   182.6 &   -27.9 &    315 &
  3495\rlap{$e$} &
  3498\rlap{$e$} &
  3506\rlap{$e$} &
  3514\rlap{$e$} &
  3516\rlap{$e$} &
  &
  &
  &
  &
  &
&   \cr
\noalign {\smallskip}
   118\rlap{$c$} &     4 &   186.2 &   -15.1 &    274 &
  1520\rlap{$e$} &
  1521 &
  1535\rlap{$e$} &
  1585\rlap{$e$} &
  &
  &
  &
  &
  &
  &
&71
  \cr
   121\rlap{$c$} &     4 &   193.3 &   -19.4 &    304 &
  1605\rlap{$e$} &
  3529\rlap{$e$} &
  3534\rlap{$e$} &
  3539\rlap{$e$} &
  &
  &
  &
  &
  &
  &
&   \cr
   124 &    34 &   195.8 &   -32.8 &    142 &
  1631 &
  1644 &
  1709 &
  1736 &
  3490\rlap{$-$} &
  3492\rlap{$e$} &
  3497\rlap{$e$} &
  3500\rlap{$e$} &
  3505\rlap{$e$} &
  3509\rlap{$-$} &
Shapley&80
  \cr
 & & & & &
  3524 &
  3528 &
  3530 &
  3532 &
  3542 &
  3548\rlap{$e$} &
  3553 &
  3554 &
  3555 &
&
  \cr
 & & & & &
  3556 &
  3558 &
  3559 &
  3560 &
  3561\rlap{$e$} &
  3562 &
  3563 &
  3564 &
  3566 &
  3570 &
&  \cr
 & & & & &
  3571 &
  3572 &
  3575 &
  3577 &
  3578 &
  &
  &
  &
  &
  &
  &
  \cr
   126 &     6 &   195.9 &    -2.3 &    241 &
  1620 &
  1650 &
  1651 &
  1663 &
  1692 &
  1750 &
  &
  &
  &
  &
  & 78
  \cr
   127 &     5 &   197.4 &   -30.4 &    217 &
  1648 &
  3531 &
  3549\rlap{$e$} &
  3552\rlap{$e$} &
  3557\rlap{$-$} &
  &
  &
  &
  &
  &
&76, 79
  \cr
   128 &     6 &   197.7 &   -33.1 &     39 &
  1060 &
  3526 &
  3537 &
  3565 &
  3574 &
  3581 &
  &
  &
  &
  &
Hydra - Centaurus &74
  \cr
   136 &     4 &   206.1 &     3.6 &    223 &
  1773 &
  1780 &
  1784 &
  1809 &
  &
  &
  &
  &
  &
  &
&82
  \cr
   138 &    12 &   209.8 &    25.4 &    196 &
  1775 &
  1781 &
  1795 &
  1800 &
  1825 &
  1827 &
  1828 &
  1831 &
  1861 &
  1873 &
Bootes&83
  \cr
 & & & & &
  1898 &
  1927 &
  &
  &
  &
  &
  &
  &
  &
  &
&  \cr
   147 &     4 &   220.6 &    54.8 &    294 &
  1925 &
  1962 &
  1999 &
  2000 &
  &
  &
  &
  &
  &
  &
&86
  \cr
   150 &    10 &   223.6 &    21.1 &    324 &
  1972 &
  1976 &
  1980 &
  1986 &
  1988 &
  1997\rlap{$e$} &
  2001 &
  2006 &
  2017 &
  2036 &
Bootes A& 
  \cr
\noalign {\smallskip}
   154 &     4 &   228.0 &     4.9 &    224 &
  2028 &
  2029 &
  2033 &
  2066 &
  &
  &
  &
  &
  &
  &
&89
  \cr
   155 &     4 &   228.4 &    -2.5 &    320 &
  2035\rlap{$e$} &
  2045\rlap{$e$} &
  2050 &
  2053 &
  &
  &
  &
  &
  &
  &
&  \cr
   157 &     6 &   229.1 &    31.7 &    323 &
  2034 &
  2046\rlap{$e$} &
  2049 &
  2062 &
  2069 &
  2083 &
  &
  &
  &
  &
  \cr
   158 &     8 &   230.8 &    29.7 &    208 &
  2019 &
  2061 &
  2065 &
  2067 &
  2079 &
  2089 &
  2092 &
  2124 &
  &
  &
Corona Borealis &90
  \cr
   160 &    12 &   236.2 &    18.5 &    105 &
  2040 &
  2052 &
  2055 &
  2063 &
  2107 &
  2147 &
  2148 &
  2151 &
  2152 &
  2162 &
Hercules&92
  \cr
 & & & & &
  2197 &
  2199 &
  &
  &
  &
  &
  &
  &
  &
  &
&  \cr
   162 &     4 &   242.2 &    51.6 &    176 &
  2149 &
  2168 &
  2169 &
  2184 &
  &
  &
  &
  &
  &
  &
&93
  \cr
     164 &     5 &   247.6 &    27.8 &    279 &
  2175 &
  2178 &
  2200 &
  2223 &
  2228 &
  &
  &
  &
  &
  &
&  \cr
   168 &     5 &   261.1 &    77.9 &    171 &
  2248 &
  2256 &
  2271 &
  2296 &
  2309 &
  &
  &
  &
  &
  &
&96
  \cr
   170 &     7 &   276.9 &    69.6 &    249 &
  2295 &
  2301 &
  2304 &
  2308 &
  2311 &
  2312 &
  2315 &
  &
  &
  &
&97
  \cr
   174 &    10 &   308.2 &   -35.0 &    259 &
  3677 &
  3681\rlap{$e$} &
  3682 &
  3690\rlap{$e$} &
  3691 &
  3693 &
  3694 &
  3695 &
  3696 &
  3705 &
Microscopium&101
  \cr
\noalign {\smallskip}
   178\rlap{$c$} &     4 &   310.2 &   -80.7 &    257 &
  3644\rlap{$e$} &
  3684\rlap{$e$} &
  3728\rlap{$e$} &
  3741\rlap{$e$} &
  &
  &
  &
  &
  &
  &
&  \cr
   182\rlap{$c$} &     4 &   319.8 &   -43.4 &    244 &
  3751\rlap{$e$} &
  3755\rlap{$e$} &
  3756 &
  3774\rlap{$e$} &
  &
  &
  &
  &
  &
  &
&  \cr
   183\rlap{$c$} &     6 &   320.6 &   -44.0 &    310 &
  3749\rlap{$e$} &
  3754\rlap{$e$} &
  3757\rlap{$e$} &
  3767\rlap{$e$} &
  3772\rlap{$e$} &
  3775 &
  &
  &
  &
  &
&  \cr
   184 &     4 &   321.7 &   -21.6 &    325 &
  2339 &
  2347 &
  3770\rlap{$e$} &
  3778 &
  &
  &
  &
  &
  &
  &
&  \cr
   188 &     9 &   327.6 &   -13.4 &    170 &
  2361 &
  2362 &
  2366 &
  2372 &
  2382 &
  2399 &
  2401 &
  2405\rlap{$e$} &
  2415 &
  &
Aquarius - Cetus&108
  \cr
   189 &     4 &   327.9 &   -19.7 &    234 &
  2370\rlap{$e$} &
  2378 &
  2394 &
  2412 &
  &
  &
  &
  &
  &
  &
Aquarius - Capricornus&111
  \cr
   190 &     5 &   328.4 &   -30.6 &    256 &
  3795 &
  3812 &
  3813 &
  3832 &
  3837 &
  &
  &
  &
  &
  &
&106, 107
  \cr
   192 &     8 &   329.8 &   -55.4 &    215 &
  3771 &
  3785 &
  3806 &
  3822 &
  3825 &
  3849 &
  3867\rlap{$e$} &
  3886 &
  &
  &
Grus - Indus& 109
  \cr
   193 &     8 &   330.5 &    -9.9 &    239 &
  2376 &
  2377 &
  2400 &
  2402 &
  2410 &
  2420 &
  2428 &
  2448 &
  &
  &
Aquarius B&113
  \cr
   197 &     9 &   336.4 &   -51.3 &    279 &
  3796\rlap{$-$} &
  3836\rlap{$e$} &
  3850\rlap{$e$} &
  3864 &
  3877 &
  3883 &
  3911 &
  3915\rlap{$e$} &
  3922 &
  &
Grus&115
  \cr
\noalign {\smallskip}
   202 &     5 &   343.5 &    17.5 &    235 &
  2458 &
  2479 &
  2516 &
  2524 &
  2564 &
  &
  &
  &
  &
  &
&119
  \cr
   205 &    19 &   346.1 &   -20.3 &    238 &
  2456 &
  2459 &
  2462 &
  2480 &
  2492 &
  2500 &
  2502\rlap{$e$} &
  2523\rlap{$e$} &
  2528 &
  2538 &
Aquarius&118, 120   \cr
 & & & & &
  2539\rlap{$e$} &
  2541 &
  2556 &
  2566 &
  2596\rlap{$e$} &
  2599 &
  2600\rlap{$e$} &
  2605\rlap{$e$} &
  3985\rlap{$e$} &
  &
& 126 \cr
   207 &     4 &   346.9 &   -14.1 &    306 &
  2529 &
  2533 &
  2543 &
  2559 &
  &
  &
  &
  &
  &
  &
&  \cr
   208 &     6 &   348.2 &   -42.0 &    257 &
  3910 &
  3963 &
  3984 &
  3987\rlap{$e$} &
  3998 &
  4010 &
  &
  &
  &
  &
Piscis - Austrinus &121
  \cr
   209 &     7 &   348.5 &   -20.6 &    317 &
  2546 &
  2548 &
  2554 &
  2579 &
  2583\rlap{$e$} &
  2586\rlap{$e$} &
  3964\rlap{$e$} &
  &
  &
  &
&  \cr
   210 &     6 &   350.4 &   -10.7 &    229 &
  2511 &
  2525 &
  2569 &
  2597 &
  2638 &
  2670 &
  &
  &
  &
  &
Aquarius A&122
  \cr
   211 &     4 &   351.7 &    15.3 &    120 &
  2572 &
  2589 &
  2593 &
  2657 &
  &
  &
  &
  &
  &
  &
Perseus - Pegasus A&123
  \cr
   213 &     6 &   353.6 &    21.9 &    188 &
  2618 &
  2622 &
  2625 &
  2626 &
  2630 &
  2637 &
  &
  &
  &
  &
Pegasus - Pisces B&125
  \cr
}}}$$
\msn
The Table 1 gives data about superclusters. Columns are as
follows: 
\msn
(1) identification number of the supercluster in the catalogue; 
$c$ stands for supercluster candidate; 
\msn 
(2) $k$ -- multiplicity of supercluster; 
\msn
(3) and (4) $\alpha$ and $\delta$ (1950) -- centre coordinates for
supercluster;
\msn
(5): distance to the supercluster centre;
\msn
(6): numbers of supercluster members from the Abell - ACO
catalogue; 
\msn
(7): identification of supercluster;
\msn
(8) identification number of supercluster with common members from
the catalogue by EETDA.  
\msn
{\it Comments to the Table.}
Supercluster center coordinates have been found as a mean value of
supergalactic $X, Y$ and $Z$ coordinates of member clusters and
then transformed to equatorial coordinates.

Clusters with estimated redshifts are
marked with $e$; clusters with measured redshifts 
that do not belong to
superclusters determined using only clusters with measured
redshifts are marked with $-$. 

{\it Note}  -- some superclusters were misordered in the Table 3
by EETDA; correct identification numbers in the column (8)
are from the Table 2 in EETDA. We thank Prof. M. Kalinkov for
turning our attention to these typos.

\vfill\eject
\end

